Quantum fields in boson star spacetime

Boson stars have been extensively studied in classical gravity, but their quantum properties remain comparatively unexplored. In this paper, we compute the quantum scalar fields and stress tensor in boson star spacetimes within the framework of semiclassical gravity. Divergences are regularized using Pauli-Villars fields, and accurate numerical results are obtained through spectral methods. Employing coherent states enables a direct comparison between the classical part of the stress tensor and the quantum fluctuation. Our results indicate that strong spacetime curvature is the primary source of large quantum effects. The renormalized quantum energy density is mostly positive but the radial pressure is negative, suggesting that classical boson star solutions require modification once quantum effects are included. Moreover, in regimes of large curvature, the quantum fluctuations can constitute a significant fraction of the total stress tensor. The methods developed here can be generalized to other compact objects and used to study their response to quantum corrections.

==> ximpleinput.tex <==

%% \newcommand{cmd}[args][default]{def}
%% \newenvironment{nam}[args][default]{begdef}{enddef}


%% Layout

\newcommand{\bmf}{\begin{mdframed}\small} \newcommand{\emf}{\end{mdframed}}

%% Lists

\newcommand{\bim}{\begin{itemize}} \newcommand{\eim}{\end{itemize}}

%% Codes

\newcommand{\bvb}{\begin{verbatim}} \newcommand{\evb}{\end{verbatim}}

%% Tables

\newcommand{\btb}[1][htbp]{\begin{table}[#1]} \newcommand{\etb}{\end{table}}

%% Figures

\newcommand{\bfg}[1][htbp]{\begin{figure}[#1]} \newcommand{\efg}{\end{figure}}

%% Colors and comments

\newcommand{\blt}{\begin{flushleft}} \newcommand{\elt}{\end{flushleft}}
\newcommand{\brt}{\begin{flushright}} \newcommand{\ert}{\end{flushright}}
% \newcommand{\comments}{}

%% Labels

\newcommand{\sect}[1]{Section~\ref{#1}} %% sec:
\newcommand{\eref}[1]{Eq.~\eqref{#1}} %% eq:
\newcommand{\enum}[1]{Point~\ref{#1}} %% pt:
\newcommand{\fig}[1]{Figure~\ref{#1}} %% fig:
\newcommand{\tab}[1]{Table~\ref{#1}} %% tab:
\newcommand{\thrm}[1]{Theorem~\ref{#1}} %% thm:
\newcommand{\foot}[1]{Footnote~\ref{#1}} %% foo:
\newcommand{\refe}[1]{Ref.~\cite{#1}} \newcommand{\refes}[1]{Refs.~\cite{#1}}

%% Equations

\newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}} %% one equation
\newcommand{\bmult}{\begin{multline}} \newcommand{\emult}{\end{multline}} %% one equation with multiple lines and one number
\newcommand{\bal}{\begin{align}} \newcommand{\eal}{\end{align}} %% multiple equations with their own numbers
\newcommand{\bald}{\begin{equation}\begin{aligned}} \newcommand{\eald}{\end{aligned}\end{equation}} %% multiple equations share one number
\newcommand{\bsubal}{\begin{subequations}\begin{align}} \newcommand{\esubal}{\end{align}\end{subequations}} %% multiple equations share a set of numbers

%% Greek letters. Section 7.5.1, Table 4.5
%% Mathematica's definitions

\newcommand{\ai}{\alpha}
\newcommand{\bi}{\beta}
\newcommand{\gi}{\gamma}
\newcommand{\di}{\delta}
\newcommand{\ei}{\epsilon}
    \newcommand{\cei}{\varepsilon}
\newcommand{\zi}{\zeta}
\newcommand{\hi}{\eta}
\newcommand{\qi}{\theta}
    \newcommand{\cqi}{\vartheta}
\newcommand{\ii}{\iota}
\newcommand{\ki}{\kappa}
\newcommand{\li}{\lambda}
\newcommand{\mi}{\mu}
% \newcommand{\ni}{\nu} %% already defined
% \newcommand{}{\xi}
\newcommand{\omi}{o}
% \newcommand{}{\pi}
    \newcommand{\cpi}{\varpi}
\newcommand{\ri}{\rho}
    \newcommand{\cri}{\varrho}
\newcommand{\si}{\sigma}
    \newcommand{\csi}{\varsigma}
\newcommand{\ti}{\tau}
\newcommand{\ui}{\upsilon}
% \newcommand{\fi}{\phi} %% already defined
    \newcommand{\cphi}{\varphi}
\newcommand{\ci}{\chi}
\newcommand{\yi}{\psi}
\newcommand{\oi}{\omega}

\newcommand{\Gi}{\Gamma}
\newcommand{\Di}{\Delta}
\newcommand{\Qi}{\Theta}
\newcommand{\Li}{\Lambda}
% \newcommand{\}{\Xi}
% \newcommand{\}{\Pi}
\newcommand{\Si}{\Sigma}
\newcommand{\Ui}{\Upsilon}
\newcommand{\Fi}{\Phi}
\newcommand{\Yi}{\Psi}
\newcommand{\Oi}{\Omega}

\newcommand{\mn}{\mu\nu}
\newcommand{\rs}{\rho\sigma}
\newcommand{\ab}{\alpha\beta}

%% Fractions and roots. Section 7.5.3

\newcommand{\f}[2]{\frac{#1}{#2}}

%% Operators. Section 7.5.5, Table 4.7

\newcommand{\n}{\nabla}
\newcommand{\p}{\partial}
\newcommand{\D}{\mathrm{D}} % \newcommand{\uD}{\,\mathrm{D}}
\renewcommand{\d}{\mathrm{d}} \newcommand{\ud}{\,\mathrm{d}}

\newcommand{\diag}{\mathrm{diag}}

%% Accents. Section 7.5.7, Table 4.9, 4.11
%% Most single-letter commands are used for text accents, see Table 2.1

\newcommand{\h}[1]{\hat{#1}}
\renewcommand{\b}[1]{\bar{#1}}
\renewcommand{\v}[1]{\vec{#1}}
\renewcommand{\t}[1]{\tilde{#1}}

\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\orv}[1]{\overleftarrow{#1}}
\newcommand{\olv}[1]{\overrightarrow{#1}}
\newcommand{\oln}[1]{\overline{#1}}
\newcommand{\uln}[1]{\underline{#1}}

%% Arrows. Section 7.5.8, Table 4.10
%% This part is ongoing

\newcommand{\lrarr}{\leftrightarrow}
\newcommand{\Larr}{\Leftarrow}
\newcommand{\Rarr}{\Rightarrow}
\newcommand{\Lrarr}{\Leftrightarrow}

%% Bracketing and delimiters. Section 7.5.9, Table 4.12

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
% \newcommand{\lro}{\left(}  \newcommand{\lpa}{\left(}  \renewcommand{\(}{\left(}
% \newcommand{\rro}{\right)} \newcommand{\rpa}{\right)} \renewcommand{\)}{\right)}
% \newcommand{\lsq}{\left(}  \newcommand{\lbr}{\left[}  \renewcommand{\[}{\left[}
% \newcommand{\rsq}{\right)} \newcommand{\rbr}{\right]} \renewcommand{\]}{\right]}
%                                                       \newcommand{}{\left\{}
%                                                       \newcommand{}{\right\}}
% \newcommand{\lan}{\left\langle}                       \renewcommand{\<}{\left\langle}
% \newcommand{\ran}{\right\rangle}                      \renewcommand{\>}{\right\rangle}

%% Math fonts
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mcl}[1]{\mathcal{#1}}
\newcommand{\msr}[1]{\mathscr{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
% \newcommand{\m}[1]{\math{#1}}
\newcommand{\bsb}[1]{\boldsymbol{#1}} %% use \bm is better





% \newcommand{\}{}


